Fully Dynamic Algorithm for Top-$k$ Densest Subgraphs

Given a large graph, the densest-subgraph problem asks to find a subgraph with maximum average degree. When considering the top-$k$ version of this problem, a na\"ive solution is to iteratively find the densest subgraph and remove it in each iteration. However, such a solution is impractical due to high processing cost. The problem is further complicated when dealing with dynamic graphs, since adding or removing an edge requires re-running the algorithm. In this paper, we study the top-$k$ densest-subgraph problem in the sliding-window model and propose an efficient fully-dynamic algorithm. The input of our algorithm consists of an edge stream, and the goal is to find the node-disjoint subgraphs that maximize the sum of their densities. In contrast to existing state-of-the-art solutions that require iterating over the entire graph upon any update, our algorithm profits from the observation that updates only affect a limited region of the graph. Therefore, the top-$k$ densest subgraphs are maintained by only applying local updates. We provide a theoretical analysis of the proposed algorithm and show empirically that the algorithm often generates denser subgraphs than state-of-the-art competitors. Experiments show an improvement in efficiency of up to five orders of magnitude compared to state-of-the-art solutions.

==> sections/Analysis.tex <==
\section{Analysis}
\label{sec:analysis}
We note that our algorithm executes in multiple iterations, where in each iteration, nodes try to perform identifier exchange to improve the social awareness in the system. 
The algorithm operates greedily to optimize the cost.
However, it is not immediately clear that the convergence of the algorithm is ever satisfied.
In this section, we show that our algorithm actually terminates in finite number of steps.
To demonstrate this, we require two different lemmas.
Absorbing states define the states of the system where most nodes are close to their friends in the identifier space or in the overlay, and no further movement of nodes is possible.
The rigorous arguments and more details can be found in \cite{7094714}.
\subsection{Lemma 1: The algorithm is a Markov Chain} 

\textit{Proof:} Our algorithm follows a chain of linked swap events, where next state depends only on the current state of the system.
Consider  at a time $t$, a node \textit{i} selects a node \textit{j} using any of the peer selection schemes.
Observe that the peer selection scheme relies on the local information of node \textit{i}. 
Then, nodes \textit{i} and \textit{j} evaluate the identifier exchange process and initiate a swap of their identifiers if the new identifiers bring gain in terms of nodes proximity. 
Therefore, the states of nodes \textit{i} and \textit{j} at time $t+1$ is a random process which depends only on the current state of a node at time \textit{t}.

\subsection{Lemma 2: The Markov chain of the the algorithm is irreducible with \texorpdfstring{$\phi$}{} being the set of absorbing states} 

\textit{Proof:} 
In order to proof this lemma, we need to show that the probability of reaching a fixed point in set of absorbing states $\phi$ is non-zero.
We prove this lemma by splitting it into two parts: first, we need to show that there exists a set $\phi$ of absorbing states. Second, we show that any state of the Markov chain is irreducible. 
Absorbing states are the node-to-identifier assignments that result in the minimum cost such that any reassignment produces a higher cost. Clearly, the existence of absorbing states is obvious as the by number of nodes and identifiers are finite. 
Irreducibility guarantees that the absorbing states are reachable by the transient, non-absorbing, states. 
 
First we show that that the Markov Chain is irreducible. 
A matrix \textit{M} is irreducible if and only if its associated graph \textit{$G_M$} is strongly connected. 
Therefore, we need to show that there is a path connecting any pair of nodes \textit{i} and \textit{j} after embedding the social graph on top of DHT overlay. 
This guarantee is provided by the Symphony identifier mapping and routing process that each node in the overlay is capable of reaching any other node in O($\dfrac{1}{k}$log(N)) steps.
Therefore, any node \textit{i} reaches another node \textit{j} by following a hop-by-hop route via intermediate nodes with identifiers closer to \textit{i} according to the distance function. 
Thus, the DHT overlay is strongly connected as there exist a path between any pair of nodes.  
 
The second part of the lemma requires a condition where, regardless of the current state, we reach any other state in a finite time. 
Our algorithm is a heuristic-based  method, where nodes select random peers and try to exchange their identifier to improve social awareness.
Specifically, there are two states of the system that are transient states and absorbing states.
The algorithm leverages the cost function, defined in the previous section, to take the identifier swapping decision. 
The nature of the cost function allows the nodes in the overlay to migrate between transient states and from any transient state to an absorbing state.
The movement between similar transient states guarantees that algorithm is never stuck in a loop and the overlay is always converging towards an absorbing state.
However, the cost function does not allow the nodes to move back from an absorbing state to a transient state.
Therefore, there is always a probability to reach one of the absorbing states in finite time.


==> sections/applications.tex <==
%% LITERATURE
\subsection{Applications}
\label{sec:app}


==> sections/problem-def.tex <==
% !TEX root =  ../project.tex
%% MODEL

%% PROBLEM DEFINITION
\section{Bounds}
\label{prob-def}


 

 

